F2former: When Fractional Fourier Meets Deep Wiener Deconvolution and Selective Frequency Transformer for Image Deblurring

Recent progress in image deblurring techniques focuses mainly on operating in both frequency and spatial domains using the Fourier transform (FT) properties. However, their performance is limited due to the dependency of FT on stationary signals and its lack of capability to extract spatial-frequency properties. In this paper, we propose a novel approach based on the Fractional Fourier Transform (FRFT), a unified spatial-frequency representation leveraging both spatial and frequency components simultaneously, making it ideal for processing non-stationary signals like images. Specifically, we introduce a Fractional Fourier Transformer (F2former), where we combine the classical fractional Fourier based Wiener deconvolution (F2WD) as well as a multi-branch encoder-decoder transformer based on a new fractional frequency aware transformer block (F2TB). We design F2TB consisting of a fractional frequency aware self-attention (F2SA) to estimate element-wise product attention based on important frequency components and a novel feed-forward network based on frequency division multiplexing (FM-FFN) to refine high and low frequency features separately for efficient latent clear image restoration. Experimental results for the cases of both motion deblurring as well as defocus deblurring show that the performance of our proposed method is superior to other state-of-the-art (SOTA) approaches.

==> Tables/keb_algorithm2.tex <==
% \begin{algorithm}[H]
% \caption{An algorithm for estimating blur kernel $\mathbf{K}$}
% \label{alg:cap}
% % \begin{algorithmic}
% \textbf{Require:} Blurry input image $\mathbf{X}$\\
% $\partial \mathbf{X} \gets \text{Conv}_{1\times 1}\left(\text{UFPdeblur}(\mathbf{X})\right)$\\
%  $\partial_v \mathbf{X}, \partial_h \mathbf{X} \gets \text{Sobel}(\partial \mathbf{X})$ \Comment{Sobel filter operation for horizontal and vertical gradient extraction}\\
% $\partial_v \mathbf{X}_e, \partial_h \mathbf{X}_e \gets f_K(\partial_v \mathbf{X}), f_K(\partial_h \mathbf{X}$) \Comment{Autoencoder operation}\\
% \textbf{for}{$i=1:\tau$}\\
%      Solve for $\mathbf{K}$ using equation \ref{eq18}\\
%     Solve for $\mathbf{X}_l$ using 2nd optimization in equation \ref{eq17}\\
%     $\partial \mathbf{X}_l \gets \text{Conv}_{1\times 1}\left(\text{UFPdeblur}(\mathbf{X}_l)\right)$\\
%      $\partial \mathbf{X}_e \gets \partial \mathbf{X}_l$
% \textbf{end for}\\
% \textbf{return} Estimated blur kernel $\mathbf{K}$
% % \end{algorithmic}
% \end{algorithm}
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Image 03-09-24 at 10.09 PM.jpg}
    \label{fig:enter-label}
\end{figure}
